A distributive lattice of model structures relating to spectral sequences

The $S$-model category structures on filtered chain complexes and bicomplexes were introduced by Cirici, Egas Santander, Livernet and Whitehouse and later generalised by this author. In this paper we show they are left proper, cellular and stable model categories. We use these properties and the Cellularization Principle of Greenlees and Shipley to show that an adjunction with right adjoint the product totalisation functor from bicomplexes to filtered chains is a Quillen equivalence. Combined with other known Quillen equivalences between filtered chains this shows these model categories all present the same homotopy category. We also construct a distributive lattice whose elements are the $S$-model categories of filtered chain complexes.

==> tex/monoidal.tex <==
\section{Monoidal model structures on $\fChS$}\label{monoidal}
\subsection{Cofibrant replacement of the unit}
In the model category structures on multicomplexes of \cite{FGLW} the authors show the unit $R^{0,0}$ is not cofibrant and give a cofibrant replacement of the form of an `infinite staircase' \cite[Example 6.6 and Proposition 6.7]{FGLW}.
Similarly in $\fChS$ we show the monoidal unit $R_{(0)}^0$ is not cofibrant and as in the case for multicomplexes our cofibrant replacement resembles an inifinite staircase.
We first construct a weakly equivalent filtered chain complex and show it is cofibrant in $\fChS$.

\begin{defi}\label{rCofibrantUnit}
  The filtered chain complex $Q_r\I$ is given by
  \begin{equation*}
    Q_r\I \coloneqq \left(\bigoplus_{i=0}^\infty R_{(-i)}^0 \longrightarrow
      \bigoplus_{j=1}^\infty R_{(-r-j)}^1\right)
  \end{equation*}
  where the differential is given for $i\geq 1$ by mapping each $R_{(-i)}^0$ diagonally onto the copies of $R$ indexed by $R_{(-i-r)}^1$ and $R_{(-i-r-1)}^1$ and for $i=0$ by mapping $R_{(0)}^0$ identically onto $R_{(-r-1)}^1$.
\end{defi}
This is more easily pictured as in 
\begin{equation*}
  \begin{tikzcd}[row sep=0.5em]
    R_{(0)}^0 \arrow[r] & R_{(-r-1)}^1 \\ 
    R_{(-1)}^0 \arrow[r] \arrow[ur] & R_{(-r-2)}^1 \\
    R_{(-2)}^0 \arrow[r] \arrow[ur] & R_{(-r-3)}^1 \\
    {\makesamewidth[c]{$_{(-1)}R_0$}{$\vdots$}} \arrow[r] \arrow[ur] &
    {\makesamewidth[c]{$_{(-r-1)}R_{-1}$}{$\vdots$}}
  \end{tikzcd}
\end{equation*}
where all arrows are identity morphisms and giving a resemblance to the infinite staircase cofibrant replacement of \cite{FGLW}.
We denote by $1_{(p)}^n$ a generator of the $R_{(p)}^n$ component of $Q_r\I$ for appropriate indices.
\begin{defi}\label{rCofibrantUnitReplacement}
  We denote by $\pi_r\colon Q_r\I\rightarrow R_{(0)}^0$ the morphism of filtered chain complexes which is the projection of $Q_r\I$ onto its $R_{(0)}^0$ component.
\end{defi}
\begin{exam}\label{QrISS}
  We consider the spectral sequence associated to $Q_r\I$.
  The $0$-page is given by $E_0^{p,p+n}=F_pQ_r\I^n/F_{p-1}Q_r\I^n$ and so there is a copy of $R$ in bidegrees $(p,p)$ for $p\leq 0$ and $(p-r,p-r+1)$ for $p\leq-1$.
  Consider then the $k$-page differential $d_k$ of bidegree $(-k,-k+1)$.
  For $k<r$ these must all be $0$ for degree reasons.
  For $k=r$ there are potentially non-zero differentials between the $R$ in bidegrees $(p,p)$ and $(p-r,p-r+1)$ for $p\leq -1$.
  We show these are all identity differentials.

  The elements $1_{(p)}^0$ are representatives for the copies of $R$ in bidegrees $(p,p)$ for $p\leq-1$ on the $r$-page.
  Its differential is given by $1_{(p-r)}^1+1_{(p-r-1)}^1$ whose image class in $E_r^{p-r,p-r+1}\cong E_0^{p-r,p-r+1}=F_{p-r}Q_r\I^1/F_{p-r-1}Q_r\I^1$ is the same as that of $1_{(p-r)}^1$ hence the $r$-page differentials from $(p,p)$ with $p\leq -1$ are identities.
\end{exam}
\begin{lemm}\label{rCofibrantUnitReplacementAcyclicFibration}
  The morphism $\pi_r$ is an $S$-acyclic fibration.
\end{lemm}
\begin{proof}
  The morphism is an $S$-fibration since the component $R_{(0)}^0$ of $Q_r\I$ is a $k$-cycle for all $k\leq r+1$.
  The discussion above shows that it is in addition an $r$-weak equivalence.
\end{proof}
We now need to show that $Q_r\I$ is cofibrant.
Note first there is a change of basis on the filtered chain complexes $\left(R_{(p)}^n\overset{\Delta}{\rightarrow} R_{(p)}^{n+1}\oplus R_{(p-1)}^{n+1}\right)$ compatible with the filtration.
By this we mean that the isomorphism exhibiting the change of basis and its inverse are morphisms of filtered chain complexes.
The change of basis is depicted as the vertical morphisms in Diagram \ref{eq:ChangeOfBasis}.
\begin{equation}
  \label{eq:ChangeOfBasis}
  \begin{tikzcd}[ampersand replacement=\&]
    \left(R_{(p)}^n\arrow[r,"\Delta"]\arrow[d,"1"]\right.\&
    \left.R_{(p)}^{n+1}\oplus R_{(p-1)}^{n+1}\right)\arrow[d,"{\begin{pmatrix}1&0\\1&-1\end{pmatrix}}"]\\
    \left(R_{(p)}^n\arrow[r,"{\begin{pmatrix}1\\0\end{pmatrix}}"]\right.\&
    \left.R_{(p)}^{n+1}\oplus R_{(p-1)}^{n+1}\right)
  \end{tikzcd}
\end{equation}
\begin{rema}
  If one writes $M\coloneqq R_{(p_1)}\oplus R_{(p_2)}\oplus\ldots\oplus R_{(p_k)}$ for some filtered $R$-module with $p_1\geq p_2\geq \ldots\geq p_k$ then a change of basis compatible with filtration is precisely a lower triangular invertible matrix.
\end{rema}
We will apply this change of basis in the proof of the following.
\begin{lemm}
  The filtered chain complex $Q_r\I$ is cofibrant in $\fChS$.
\end{lemm}
\begin{proof}
  Consider a lifting problem of $Q_r\I$ against an $S$-acyclic fibration $f\colon E\rightarrow B$ as in
  \begin{equation*}
    \begin{tikzcd}
      &E\arrow[d,"f",two heads, "\sim"']\\
      Q_r\I\arrow[ur, dashed, "h"]\arrow[r]&B
    \end{tikzcd}\;.
  \end{equation*}
  We will begin by lifting the subcomplex $R_{(0)}^0\rightarrow R_{(-r-1)}^1$ of $Q_r\I$ and then inductively lift the subdiagrams $R_{(-p)}^0\overset{\Delta}{\rightarrow} R_{(-p-r)}^1\oplus R_{(-p-r-1)}^1$ subject to already having a lift for the $R_{(-p-r)}^1$ component.
  This inductive stage will make use of the change of basis.

  The subcomplex $R_{(0)}^0\rightarrow R_{(-r-1)}^1$ is a copy of $\Z_{r+1}(0,0)$ and so since $f$ is an $S$-acyclic fibration there exists a lift of this $(r+1)$-cycle. Consider now the lifting problem
  \begin{equation*}
    \begin{tikzcd}
      R_{(-p-r)}^1\arrow[d,"i"']\arrow[r]
      &E\arrow[d,"f",two heads, "\sim"']\\
      \left(R_{(-p)}^0\overset{\Delta}{\rightarrow} R_{(-p-r)}^1\oplus R_{(-p-r-1)}^1\right)
      \arrow[ur, dashed, "h_p"]\arrow[r]&B
    \end{tikzcd}
  \end{equation*}\todo{shorten arrow}
  where $i$ is the inclusion of the $R_{(-p-r)}^1$ component.
  Applying the filtered change of basis outlined above converts this diagram to an isomorphic one of the form
  \begin{equation*}
    \begin{tikzcd}
      R_{(-p-r)}^1\arrow[d,"\Delta"']\arrow[r]
      &E\arrow[d,"f",two heads, "\sim"']\\
      \left(R_{(-p)}^0\overset{i_1}{\rightarrow} R_{(-p-r)}^1\oplus R_{(-p-r-1)}^1\right)
      \arrow[ur, dashed, "h_p"]\arrow[r]&B
    \end{tikzcd}
  \end{equation*}\todo{shorten arrow}
  for which a lift $h_p$ exists: the morphism $f$ is an $S$-acyclic cofibration and the morphism $\Delta$ is a particular case of $\phi\colon \Z_{r+1}(-p-r,1)\rightarrow\B_{r+1}(-p-r,1)$ in which the images of the $R_{(-p-2r-1)}^2$ components are $0$.
  One then inducts `down the staircase step by step' using these change of bases to construct a lift $h$ of $Q_r\I$ from the individual lifts $h_p$ of the subcomplexes of $Q_r\I$.
\end{proof}
Our cofibrant replacement $Q_r\I$ of the unit then does not actually depend on all elements of $S$, only its maximum.
Note too that $Q_r\I$ being cofibrant demonstrates our subclass of cofibrant objects of $\fChr$ of \todo{ref} is indeed a strict subclass as it does not satisfy the bounded filtration condition.
\begin{lemm}
  The unit $R_{(0)}^0$ of the monoidal structure on $\fCh$ is not cofibrant.
\end{lemm}
\begin{proof}
  Consider the lifting problem
  \begin{equation*}
    \begin{tikzcd}
      & Q_r\I\arrow[d,"\pi_r", two heads, "\sim"']\\
      R_{(0)}^0\arrow[r, "1"]& R_{(0)}^0
    \end{tikzcd}
  \end{equation*}
  in which the morphism $\pi_r$ is that of \cref{rCofibrantUnitReplacement} and so by \cref{rCofibrantUnitReplacementAcyclicFibration} is an $S$-acyclic fibration.
  If a lift were to exist in this diagram then the image of $R_{(0)}^0$ in $Q_r\I$ would have to land in infinitely many summands of the cohomological degree $0$ part $\bigoplus_{p\leq 0} R_{(-p)}^0$ of $Q_r\I$ for its differential to remain $0$.
  This is not possible by definition of the coproduct.
  Hence no lift can exist and so $R_{(0)}^0$ is not cofibrant. 
\end{proof}
\subsection{The unit axiom}
We will demonstrate the unit axiom holds in $\fChS$, in fact we demonstrate the very strong unit axiom holds.
We begin by describing cycle and boundary objects in $Q_r\I\otimes A$ for an $A\in\fCh$.
Recall the notation $1_{(p)}^n$ for the generators of the summands $R_{(p)}^n$ of $Q_r\I$ of \cref{QrISS}.
An element $q\in F_p\left(Q_r\I\otimes A\right)^n$ can be written as a finite sum of tensors:
\begin{equation}\label{qOfProduct}
  q = \sum_{k\geq 0}1_{(-k)}^0 \otimes a_{(p+k)}^n +
  \sum_{j\geq 0} 1_{(-j-r-1)}^1 \otimes a_{(p+j+r+1)}^{n-1}
\end{equation}
where $a_{(p)}^n\in F_pA^n$.
The differential $d=d^{Q_r\I\otimes A}$ of the monoidal product of $Q_r\I$ and $A$ applied to $q$ is given by:
\begin{equation*}
  dq = \sum_{k\geq 0}1_{(-k)}^0\otimes da_{(p+k)}^n + \sum_{j\geq 0}1_{(-j-r-1)}^1\otimes
  \left(-da_{(p+j+r+1)}^{n-1}+a_{(p+j)}^n+a_{(p+j+1)}^n\right)
\end{equation*}
We now give a description of the $(r+1)$-cycles of $Q_r\I\otimes A$.
\todo{do I want a proof of this?}
\begin{lemm}\label{QrIACycles}
  Let $q\in F_p(Q_r\I\otimes A)$ be given as in \cref{qOfProduct}, then $q\in Z_{r+1}^{p,p+n}(Q_r\I\otimes A)$ if and only if the following hold:
  \begin{enumerate}
  \item $a_{(p)}^n\in Z_{r+1}^{p,p+n}(A)$, 
  \item $a_{(p+k)}^n\in B_{r+1}^{p+k,p+k+n}(A)$, for each $k\geq 1$, and
  \item $a_{(p+k)}^n-da_{(p+r+k)}^{n-1}\in F_{p-1+k}A^n$, for each $k\geq1$.\qed
  \end{enumerate}
\end{lemm}
\todo{do I want a proof of this?}
\begin{lemm}\label{QrIABoundaries}
  Let $q\in F_p(Q_r\I\otimes A)$ be given as in \cref{qOfProduct}, then $q\in B_{r+1}^{p,p+n}(Q_r\I\otimes A)$ if and only if $q$ satisfies:
  \begin{enumerate}
  \item $a_{(p)}^n\in B_{r+1}^{p,p+n}(A)$, 
  \end{enumerate}
  as well as conditions 2 and 3 from \cref{QrIACycles}.\qed
\end{lemm}
Note that in the above lemmas condition $3$ is giving an explicit representation of $a_{(p+k)}^n$ as an $(r+1)$-boundary of $A$ so that in fact $3 \Rightarrow 2$.
\begin{prop}\label{VeryStrongUnitAxiomForFCHS}
  The morphism $\pi_r\colon Q_r\I\overset{\sim}{\twoheadrightarrow} R_{(0)}^0$ of \cref{rCofibrantUnitReplacement} satisfies the very strong unit axiom in $\fChS$.
\end{prop}
\begin{proof}
  We must show the composite morphism $Q_r\I\otimes X\rightarrow \I\otimes X\rightarrow X$ is a weak equivalence for all (not necessarily cofibrant) $X$, i.e.\ that the map
  \begin{equation}\label{QrIAMaprPage}
    E_{r+1}^{p,p+n}(Q_r\I\otimes A)= \frac{Z_{r+1}^{p,p+n}(Q_r\I\otimes A)}{B_{r+1}^{p,p+n}(Q_r\I\otimes A)}
    \longrightarrow\frac{Z_{r+1}^{p,p+n}(A)}{B_{r+1}^{p,p+n}(A)}=E_{r+1}^{p,p+n}(A)
  \end{equation}
  is an isomorphism.
  Note that \cref{QrIAMaprPage} is surjective by surjectivity of $Z_{r+1}^{p,p+n}(Q_r\I\otimes A)\rightarrow Z_{r+1}^{p,p+n}(A)$: for any $(r+1)$-cycle $a$ of $A$ it is the image of $1_{(0)}^0\otimes a$ which is itself an $(r+1)$-cycle of $Q_r\I\otimes A$.

  For injectivity let $q\in \Z_{r+1}^{p,p+n}(Q_r\I\otimes A)$ be of the form \cref{qOfProduct} and such that its image under $Q_r\I\otimes A\rightarrow A$ is a boundary, i.e.\ $a_{(p)}^n\in B_{r+1}^{p,p+n}(A)$.
  We pick an explicit representation of $a_{(p)}^n$ as a boundary, say $da_{(p+r)}^{n-1}+a_{(p-1)}^n$ where these $a_{(\ast)}^\ast$ were not specified previously in $q$.
  Recall too from \cref{QrIACycles} that condition $3$ gave explicit representatives, for $k\geq 1$, for $a_{(p+k)}^n$ as $(r+1)$-boundaries: $a_{(p+k)}^n=da_{(p+r+k)}^{n-1}+b_{(p-1+k)}^n$. For convenience write $b_{(p-1)}^{n}\coloneqq a_{(p-1)}^{n}$.

  For $k\geq 0$ we have the following equality:
  \begin{align}\label{BoundaryElementApkn}
    1_{(-k)}^0\otimes a_{(p+k)}^n &= d\left(1_{(-k)}^0\otimes a_{(p+k+r)}^{n-1}\right) +1_{(-k)}^0\otimes b_{(p+k-1)}^n\nonumber\\
                                  & \phantom{--}-1_{(-k-r)}^1\otimes a_{(p+k+r)}^{n-1}-1_{(-k-r-1)}^1\otimes a_{(p+k+r)}^{n-1}
  \end{align}
  where the penultimate term is interpreted as $0$ if $k=0$.
  Rearranging \cref{BoundaryElementApkn} and summing over $k\geq 0$ gives:
  \begin{align*}
    q &= \sum_{k\geq0}\left(1_{(-k)}^0\otimes a_{(p+k)}^n+1_{(-k-r)}^1\otimes a_{(p+k+r)}^{n-1}\right)\\
      &= \sum_{k\geq0}\left(d\left(1_{(-k)}^0\otimes a_{(p+k+r)}^{n-1}\right)+1_{(-k)}^0\otimes b_{(p+k-1)}^n
        -1_{(-k-r-1)}^1\otimes a_{(p+k+r)}^{n-1}\right)\;.
  \end{align*}
  We now identify terms in this second expression for $q$. The terms of the form $d\left(1_{(-k)}^0\otimes a_{(p+k+r)}^{n-1}\right)$ are $d$ applied to an element of $Z_{r}^{p+r,p+r+n-1}(Q_r\I\otimes A)$ and those of the form $1_{(-k)}^0\otimes b_{(p+k-1)}^n-1_{(p+k-1)}^1\otimes a_{(p+k+r)}^{n-1}$ are elements of $Z_{r}^{p-1,p-1+n}(Q_r\I\otimes A)$. We have then written $q$ as an element of $B_{r+1}^{p,p+n}(Q_r\I\otimes A)$. This shows injectivity of \cref{QrIAMaprPage}.
\end{proof}
\subsection{The pushout-product axiom}
We turn our attention now to verifying the pushout-product axiom of \cref{monoidalModelCategory}.
Recall from \cref{PushoutProductOnGeneratingCofibrations} that, since the $\fChS$ are symmetric monoidal and cofibrantly generated, we need only check that $I_S\boxtimes I_S\subseteq I_S\Cof$, $I_S\boxtimes J_S\subseteq J_S\Cof$ and $J_S\boxtimes J_S\subseteq J_S\Cof$.
The latter two conditions will be easily checked the first however is a somewhat involved computation.
The following lemmas prove the two conditions involving $J_S$.

\begin{lemm}\label{PushoutProductOfJAndJIsAcyclicCofibration}
  Let $s\leq t$. There is an isomorphism of filtered chain complexes:
  \begin{equation*}
    \Z_t(q,m)\otimes\Z_s(p,n)\cong \Z_s(p+q,n+m)\oplus\Z_s(p+q-t,n+m+1)\;\pushQED{\qed}\qedhere
  \end{equation*}
\end{lemm}
\begin{lemm}\label{PushoutProductOfIAndJIsAcyclicCofibration}
  Let $s\leq r$. There is an isomorphism of morphisms of filtered chain complexes between the pushout-product:
  \begin{equation*}
    \begin{pmatrix}
      \Z_{r+1}(p,n)\\\downarrow\\\B_{r+1}(p,n)
    \end{pmatrix}\boxtimes
    \begin{pmatrix}
      0\\\downarrow\\\Z_s(q,m)
    \end{pmatrix}\cong
    \begin{pmatrix}
      \Z_{r+1}(p,n)\otimes\Z_s(q,m)\\
      \downarrow\\
      \B_{r+1}(p,n)\otimes\Z_s(q,m)
    \end{pmatrix}
  \end{equation*}
  and the direct sum of morphisms:
  \begin{align*}
    \begin{pmatrix}
      0\\\downarrow\\Z_s(p+q+r,n+m-1)
    \end{pmatrix}&\oplus
                   \begin{pmatrix}
                     0\\\downarrow\\\Z_s(p+q-1,n+m)
                   \end{pmatrix}\\
                 &\oplus
                   \begin{pmatrix}
                     \Z_s(p+q-r-1,n+m+1)\\\downarrow\\\Z_s(p+q-r-1,n+m+1)
                   \end{pmatrix}\\
                 &\oplus
                   \begin{pmatrix}
                     \Z_s(p+q,n+m)\\\downarrow\\\Z_s(p+q,n+m)
                   \end{pmatrix}\;.
  \end{align*}
\end{lemm}
\begin{proof}
  The proof is \todo{write appendix proof}.
\end{proof}
These lemmas prove the following.
\begin{coro}
  In the model category $\fChS$ morphisms of the pushout-products $I_S\boxtimes J_S$ and $J_S\boxtimes J_S$ are elements of $J_S\Cof$.\qed
\end{coro}
The case $I_S\boxtimes I_S\subseteq I_S$ involves computing pushouts in filtered chains.
Recall there is an adjunction $\inadj{\rho}{\Ch^{\Zbb_+}}{\fCh}{i}$ and by \cref{FilteredChainsLimits} we can instead compute colimits in the functor category $\Ch^{\Zbb_+}$.
Given a diagram $X\colon \mc{J}\rightarrow\fCh$ its colimit is given by $\rho\colim_{\mc{J}}iX$.
\begin{prop}\label{pushoutProductOfGeneratingCofibrations}
  The pushout-product of $i\colon\Z_{r+1}(p,n)\rightarrow\B_{r+1}(p,n)$ and $j\colon\Z_{r+1}(q,m)\rightarrow\B_{r+1}(q,m)$ is given as in \cref{PushoutProductOfIandI}.
\end{prop}
\begin{proof}
  The proof is in \todo{appendix proof}.
\end{proof}
\begin{figure}[h]
  \begin{equation*}
    \begin{tikzcd}[column sep=1cm]
      %% Begin first diagram
      &R_{(p+r)+(q)}^{n+m-1} \arrow[r,"(-1)^{n-1}"]\arrow[d,"\alpha"]&R_{(p+r)+(q-r-1)}^{n+m}\arrow[d,"i_1"] \\
      R_{(p)+(q+r)}^{n+m-1}\arrow[d,"1"]\arrow[r,"\beta"]&
      \begin{matrix}R_{(p)+(q)}^{n+m}\amsamp\oplus\amsamp R_{(p)+(q-1)}^{n+m}\\
        \oplus\amsamp\amsamp\\R_{(p-1)+(q)}^{n+m}\end{matrix}\arrow[r,"\epsilon"]\arrow[d,"\gamma"]&
      \begin{matrix}R_{(p)+(q-r-1)}^{n+m+1}\\\oplus\\ R_{(p-1)+(q-r-1)}^{n+m+1}\end{matrix}\arrow[d,"\pi_2"]\\
      R_{(p-r-1)+(q+r)}^{n+m}\arrow[r,"(-1)^{n+1}i_1"]&
      \begin{matrix}R_{(p-r-1)+(q)}^{n+m+1}\amsamp\oplus\amsamp R_{(p-r-1)+(q-1)}^{n+m+1}\end{matrix}\arrow[r,"(-1)^{n+1}\pi_2"]
      \arrow[ddd, "i\boxtimes j", dashed]
      &R_{(p-r-1)+(q-r-1)}^{n+m+2}\\\\\\
      %% Begin second diagram
      R_{(p+r)+(q+r)}^{(n-1)+(m-1)}\arrow[r,"(-1)^{n-1}i_1"]\arrow[d,"i_1"]
      &\begin{matrix}R_{(p+r)+(q)}^{(n-1)+(m)}
        \amsamp\oplus\amsamp R_{(p+r)+(q-1)}^{(n-1)+(m)}\end{matrix}
      \arrow[r,"(-1)^{n-1}\pi_2"]\arrow[d]
      &R_{(p+r)+(q-r-1)}^{(n-1)+(m+1)}\arrow[d,"1_1"]\\
      \begin{matrix}R_{(p)+(q+r)}^{(n)+(m-1)}\\\oplus\\R_{(p-1)+(q+r)}^{(n)+(m-1)}\end{matrix}
      \arrow[r,"(-1)^n"]\arrow[d,"\pi_2"]&
      \begin{matrix}R_{(p)+(q)}^{(n)+(m)}\amsamp\oplus\amsamp R_{(p)+(q-1)}^{(n)+(m)}
        \\\oplus\amsamp\amsamp\oplus\\
        R_{(p-1)+(q)}^{(n)+(m)}\amsamp\oplus\amsamp R_{(p-1)+(q-1)}^{(n)+(m)}\end{matrix}
      \arrow[r,"(-1)^n"]\arrow[d]
      &\begin{matrix}R_{(p)+(q-r-1)}^{(n)+(m+1)}\\\oplus\\R_{(p-1)+(q-r-1)}^{(n)+(m+1)}\end{matrix}
      \arrow[d,"\pi_2"]\\
      R_{(p-r-1)+(q+r)}^{(n+1)+(m-1)}\arrow[r,"(-1)^{n+1}i_1"]&
      \begin{matrix}R_{(p-r-1)+(q)}^{(n+1)+(m)}\amsamp\oplus\amsamp R_{(p-r-1)+(q-1)}^{(n+1)+(m)}\end{matrix}
      \arrow[r,"(-1)^{n+1}\pi_2"]&
      R_{(p-r-1)+(q-r-1)}^{(n+1)+(m+1)}
    \end{tikzcd}
  \end{equation*}\caption{The pushout-product of generating cofibrations $i$ and $j$}\label{PushoutProductOfIandI}
\end{figure}
\begin{coro}\label{PushoutProductOfIAndIIsCofibration}
  The pushout-product of generating cofibrations $i\colon\Z_{r+1}(p,n)\rightarrow\B_{r+1}(p,n)$ and $j\colon\Z_{r+1}(q,m)\rightarrow\B_{r+1}(q,m)$ is a cofibration in $\fChS$.
\end{coro}
\begin{proof}
  \todo{prove}
\end{proof}
\subsection{Monoidal model categories}
\begin{theo}\label{fChSIsMonoidal}
  The model categories $\fChS$ are closed symmetric monoidal model categories.
\end{theo}
\begin{proof}
  We must show the unit and pushout-product axioms of \cref{monoidalModelCategory}.
  The unit axiom was proved in \cref{VeryStrongUnitAxiomForFCHS}.
  The pushout-product axiom was proved for $I_S\boxtimes I_S\subseteq I_S\Cof$ in \cref{PushoutProductOfIAndIIsCofibration}, for $I_S\boxtimes J_S\subseteq J_S\Cof$ in \cref{PushoutProductOfIAndJIsAcyclicCofibration} and for $J_S\boxtimes J_S\subseteq J_S\Cof$ in \cref{PushoutProductOfJAndJIsAcyclicCofibration}.
\end{proof}
Write $Q\colon \fChS\rightarrow \fChS$ for a cofibrant replacement functor.
\begin{coro}
  The homotopy category $\Ho(\fChS)$ has an induced closed symmetric monoidal structure with monoidal product given by:
  \begin{equation*}
    A\Lotimes B\coloneqq QA\otimes QB\;,
  \end{equation*}
  and internal hom object functor:
  \begin{equation*}
    R\Hom(A,B) \coloneqq \Hom(QA,B)\;.
  \end{equation*}
  We need not fibrantly replace $B$ in the hom objects since all objects of $\fChS$ are fibrant. The unit in the homotopy category is given by any cofibrant replacement of $R_{(0)}^0$, in particular we can take $Q_r\I$ from \cref{rCofibrantUnit}.
\end{coro}
\begin{proof}
  This follows from \cite[Theorem 4.3.2]{H} applied to the closed symmetric monoidal model category $\fChS$ of \cref{fChSIsMonoidal}.
\end{proof}
%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../main"
%%% End:

